From the Least to the Most: Building a Plug-and-Play Visual Reasoner via Data Synthesis

We explore multi-step reasoning in vision-language models (VLMs). The problem is challenging, as reasoning data consisting of multiple steps of visual and language processing are barely available. To overcome the challenge, we first introduce a least-to-most visual reasoning paradigm, which interleaves steps of decomposing a question into sub-questions and invoking external tools for resolving sub-questions. Based on the paradigm, we further propose a novel data synthesis approach that can automatically create questions and multi-step reasoning paths for an image in a bottom-up manner. Our approach divides the complex synthesis task into a few simple sub-tasks, and (almost entirely) relies on open-sourced models to accomplish the sub-tasks. Therefore, the entire synthesis process is reproducible and cost-efficient, and the synthesized data is quality guaranteed. With the approach, we construct $50$k visual reasoning examples. Then, we develop a visual reasoner through supervised fine-tuning, which is capable of generally enhancing the reasoning abilities of a wide range of existing VLMs in a plug-and-play fashion. Extensive experiments indicate that the visual reasoner can consistently and significantly improve four VLMs on four VQA benchmarks. Our code and dataset are available at https://github.com/steven-ccq/VisualReasoner.

==> latex/data_quality.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[!tbp]
\begin{tabular}{@{}ccc@{}}
\toprule
\textbf{Sub-Question} & \textbf{Main-Question} & \textbf{Argument} \\ \midrule
581 / 581             & 200 / 200              & 581/ 581          \\ \bottomrule
\end{tabular}
\caption{Data Quality Assessment}
\label{table:data_quality}
\end{table}
